Small Language Models: Survey, Measurements, and Insights

Small language models (SLMs), despite their widespread adoption in modern smart devices, have received significantly less academic attention compared to their large language model (LLM) counterparts, which are predominantly deployed in data centers and cloud environments. While researchers continue to improve the capabilities of LLMs in the pursuit of artificial general intelligence, SLM research aims to make machine intelligence more accessible, affordable, and efficient for everyday tasks. Focusing on transformer-based, decoder-only language models with 100M-5B parameters, we survey 70 state-of-the-art open-source SLMs, analyzing their technical innovations across three axes: architectures, training datasets, and training algorithms. In addition, we evaluate their capabilities in various domains, including commonsense reasoning, mathematics, in-context learning, and long context. To gain further insight into their on-device runtime costs, we benchmark their inference latency and memory footprints. Through in-depth analysis of our benchmarking data, we offer valuable insights to advance research in this field.

==> fig-acc-fine-tune.tex <==
\begin{figure}[h]
	\centering
	\includegraphics[width=0.7\textwidth]{figs/acc-finetune.pdf}
%  \vspace{-10pt}	
	\caption{
        SLM performance after finetuneing vs LLaMA finetuning.
		}
	\label{fig:acc-finetune}
\end{figure}

==> figs-cost/fig_memory_vs_parameters.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{figs-cost/memory_usage_vs_parameters.pdf}
    \caption{Memory Usage with Different Parameters. \mwx{merge it with Fig 7 and put them in the same page (legend can be shared).}}
    \label{fig:memory_usage_vs_parameters}
\end{figure}

==> sec-innovation.tex <==
\section{SLM Innovations: Architecture, Dataset, and Algorithms}







==> todo.tex <==
\mwx{TODO (by Dec. 1st):}

\begin{itemize}
    \item Xiang: Add instructed models and the experiments (e.g., long context via ``lost in the haystack'').
    \item Xiang: Add mobile-specific tasks, e.g., function call
    \item Zhenyan: Add a section to survey the literature on optimizing on-device SLM deployment. Refer to ``On-Device Language Models: A Comprehensive Review''.
    \item Add compressed language models part: sheared-llama, minima, gemma-2-2b, minitron-4b.
    \item Add non-transformer model part: zamba2-mini, zamba2-small.
    \item Add new models: Llama3.2, AMD-Llama-135m, CT-LLM and MAP-Neo, PhoneLM.
    \item Add chatting examples for instructed models. For example, selecting 10 interesting prompts, and show the response of each instructed SLM. This can be put in the appendix.

\end{itemize}
